Generating Comprehensive Data with Protocol Fuzzing for Applying Deep Learning to Detect Network Attacks

Network attacks have become a major security concern for organizations worldwide and have also drawn attention in the academics. Recently, researchers have applied neural networks to detect network attacks with network logs. However, public network data sets have major drawbacks such as limited data sample variations and unbalanced data with respect to malicious and benign samples. In this paper, we present a new approach, protocol fuzzing, to automatically generate high-quality network data, on which deep learning models can be trained. Our findings show that fuzzing generates data samples that cover real-world data and deep learning models trained with fuzzed data can successfully detect real network attacks.

==> 6-evaluation.tex <==
\section{Interpreting Why the Detection Models Achieved High Detection Accuracy}
\label{sec:eva}

The results presented in the previous section show that the trained (network attack detection) models have achieved high detection accuracy, as measured by metrics such as 
accuracy score, F1 score, and false positive rate. 
In this section, we would like to provide a few domain-specific interpretations on why the detection models could achieve high detection accuracy. 
In particular, we seek to answer two research questions: (1) Whether fuzzed packet fields indeed influence model accuracy? (2) Whether the protocol fuzzing approach has the ability to generate comprehensive data?    

% In this paper, we make the following hypothesis: our new method, protocol fuzzing, can help generate data to train neural networks for some network attacks' identification. In order to prove this, in this section, we will first show that real-world data are \textbf{covered by} data generated by protocol fuzzing. Second, we will prove that models trained with the protocol fuzzing generated data can identify real-world attacks.

%=====================

\subsection{Influence of Fuzzed Packet Fields on Detection  Accuracy}
\label{subsec:influential}

One of the problems we are curious about is how influential the fuzzed fields are to the accuracy of the trained neural networks. To answer this question, we have leveraged {\em permutation feature importance} \cite{breiman2001random}, a widely-adopted procedure to make machine learning more interpretable, to measure the increase or decrease in the accuracy of the model after we permute a particular feature's values. We obtained the permutation feature importance 
measurements for ARP poisoning and TELNET session hijacking identification. For DNS cache poisoning, 
we visualized the learned features in the first convolutional layer, which provide insights about which pixels of the ``image'' are emphasized.

Permutation feature importance is a model inspection technique that can be used for fitted models. It is defined as the decrease in a model score, which is the F1 score in our experiments, when a single feature value is randomly shuffled~\cite{breiman2001random}. This technique benefits from being model agnostic and can be calculated many times with different permutations of the feature, and is often used to inspect how influential some features are to the model in various deep learning applications~\cite{galkin2018human,liu2020deep,zamani2019pm2}. The drawback is that, when several features are correlated, the measurement becomes inaccurate. Our results show that, for ARP poisoning, the top three most influential features (bytes) all belong to fuzzed fields, which are \texttt{destination MAC address}, \texttt{target MAC address}, and \texttt{target IP address}; for TELNET session hijacking, one of the three most influential features is fuzzed, which are \texttt{timestamp value}, \texttt{timestamp echo reply}, and \texttt{urgent pointer}, and \texttt{urgent pointer} is fuzzed.


In summary, our experiments show that the 3 most influential features for each of the trained models usually involve one or more fuzzed packet fields. However, as for the CNN for DNS cache poisoning identification, the fuzzed field, \texttt{time to live} value in the \texttt{IP} layer, is one of the fields that are least influential.
Although our experiments show no fuzzed field is most influential on the first layer (of the model) in detecting DNS cache poisoning, the possibility that a fuzzed field is most influential on a deeper layer is not denied either. 
%show that all the fuzzed fields are most influential to the model, there is no all rounded approach to measure the feature importance, and the ways we chose, though commonly used, have their drawbacks as well. 
Deep learning models are still mostly ``black boxes''. Furthermore, not all fuzzed fields may be presented in the data samples. For example, for PtH, the fields used in the mapping (and embedding) do not concern any fuzzed fields.
% for DNS cache poisoning, all fuzzed fields but one do not present in the data sample. 
Another possibility is that, though some fuzzed fields' influences are not directly reflected from our measurements above, the fuzzed fields may affect other fields, which are in turn influential to the models. 

%============================
\subsection{Can Protocol Fuzzing Generate Comprehensive Training Data?}

A comprehensive training data set is a key factor in many 
successful applications (e.g., image classification) of deep learning. 
However, how to formally assess the comprehensiveness of the training data in deep-learning-based detection of network attacks is an issue largely 
neglected in the literature. 
In this subsection, we seek to take the first step towards 
systematically addressing this issue. 
In particular, we introduce a new notion, called \textbf{``covered-by"}, 
to capture an inherent connection between protocol fuzzing and 
training-data comprehensiveness.

The intuition behind this notion is as follows. 
First, 
a network packet is essentially a set of fields. 
Although real-world packets are usually not byte-to-byte identical to 
the packets generated through protocol fuzzing, the content  
in a particular field of a real-world packet may be identical to 
the corresponding field of a fuzzed packet. 
% Protocol fuzzing is supposed to mutate the content of only a subset of packets fields; 
Hence, it seems appropriate to do field-content-based data 
comprehensiveness assessment. 
Second, one major advantage of deep learning 
is that it requires less feature engineering than conventional 
machine learning techniques (e.g., Support Vector Machines). 
Accordingly, although a data sample in the training set 
involves the information from multiple fields, the deep learning
algorithm typically treats each element (e.g., a byte or a pixel) in 
the data sample in 
a unified way, and does not pre-extract semantic-carrying features. 
Based on this observation, we do not assess data comprehensiveness
based on a space of semantic-carrying features. 
%For example, the proposed protocol fuzzing method does not intend to enumerate all the possible real-world IP addresses. Hence, the notion of \textbf{``covered by''} should not be defined as identical at packet bytes level.
%Second, because the trained neural networks are largely a black-box with limited interpretability, we usually do not completely know the set of features used, or the exact roles played by each feature. Hence, the notion of \textbf{``covered by''} should not be defined based on features. 
%Third, since different deep learning algorithms can process network packets in very different ways, we believe that the notion of {\em covered-by} should be defined in an algorithm-specific way.

Based on the above intuition, we define the 
notion of ``covered-by" as follows:  
\begin{itemize}
\item When a real-world network packet is being ``examined" 
by a deep learning model, it will need to be firstly transformed 
to a data sample $a$ (or a portion of $a$) expected by the model. 
An element in the data sample is {\em covered-by} 
a data sample $b$ generated through the proposed protocol fuzzing method
if (1) the element's content is identical to the corresponding
element in $b$, (2) the 
packet field used to derive 
the element in $a$ has the same content as the  
field used to derive the corresponding element in $b$, 
and (3) the above-mentioned packet field is a being-fuzzed
field in the proposed protocol fuzzing.  
Note that since the definition 
intends to capture an inherent connection between protocol fuzzing
and data comprehensiveness, it ignores the elements that are 
not derived from a being-fuzzed field.  
%Here, we assume that the network packets generated by the proposed protocol fuzzing method are transformed to 
\item Given a set of data samples $S_1$ (generated through real-world network packets)    
and a training set of data samples $S_2$ generated through 
the proposed protocol fuzzing method,  
the {\em coverage rate} is defined as the ratio of $x$ to $(x+y)$. 
Here $x$ is the total number of the elements in $S_1$ 
that are covered-by one or more data samples in $S_2$. 
And $y$ is the total number of the elements in 
$S_1$ that are derived from a being-fuzzed field 
but not covered-by any data sample in $S_2$. 
\end{itemize} 

It should be noticed that coverage rate is not applicable to 
the deep learning algorithms that  
employ a mapping from an entire network packet to 
a type assigned with a particular type number. 
Accordingly, because such a mapping is done
when detecting PtH, we should not use 
coverage rate to 
measure the comprehensiveness of the training data 
generated for detecting PtH. 

%If a real-world (non-fuzzed) data sample is \textbf{bytes ``covered by''} fuzzed data samples, then, for all the fuzzed bytes or features that are mapped from fuzzed bytes presented in the real-world data sample, there exists a perfect match for each of them in the fuzzed data samples.

% Below we will propose two ways to define \textbf{``covered by''}, with respect to the two kinds of data samples as discussed in section~\ref{sec:detect_with_NN}, which is processed by two types of algorithms. 

%In the first definition, \textbf{bytes ``covered by''}, we assume that bytes in the original network packets can be inferred from the post-processing data samples. The bytes can either be directly inferred, which means that data samples directly hold the bytes values, or be indirectly inferred, which means that there exists a mapping from byte(s) to some features in the data samples.

%\theoremstyle{definition}
%\label{def:bytes-covered-by}
%\begin{definition}{\textbf{Bytes ``covered by'':}}
%    Assume that bytes in the original network packets can be inferred from the post-processing data samples. If a real-world (non-fuzzed) data sample is \textbf{bytes ``covered by''} fuzzed data samples, then, for all the fuzzed bytes or features that are mapped from fuzzed bytes presented in the real-world data sample, there exists a perfect match for each of them in the fuzzed data samples.
%\end{definition}

%Definition 1 above accounts for three network attacks in this paper, which are ARP poisoning, DNS cache poisoning, and TELNET session hijacking. In all the three attack identifications, the data samples directly hold the byte values from network packets. However, it does not suit PtH identification. Definition 1 has one pre-assumption, which is that fuzzed field(s) can be inferred directly or indirectly from the data sample, and that does not hold for PtH. As discussed in subsection~\ref{subsec:data-gen_PtH}, each data sample is a sequence of packet type numbers, and the packet type numbers are mapped from certain fields that are not fuzzed. Therefore, the data samples do not present any of the fuzzed fields. In another word, the mapping from packet fields to packet type numbers does not involve any fuzzed fields. In this case, though protocol fuzzing generated bytes are not reflected in the data sample, the order of packet type numbers is affected. Thus, in addition to definition 1, which focuses on bytes, below we present the definition of \textbf{mapping ``covered by''}, which accounts for PtH:

%\theoremstyle{definition}
%\label{def:mapping-covered-by}
%\begin{definition}{\textbf{Mapping ``covered by'':}}
 %   Assume that all features in the data samples are mapped from non-fuzzed fields. If a real-world (non-fuzzed) data sample is \textbf{Mapping ``covered by''} fuzzed data samples, then there exists a same mapping in the fuzzed data. In another word, there exists a fuzzed original network packet that has the same values as those of the real-world (non-fuzzed) network packet in the fields which are used in the mapping.
%\end{definition}

%Based on the above definition, we define a measurement of how complete real-world data are covered by data generated by protocol fuzzing as follows:
%\theoremstyle{definition}
%\label{def:coverage-rate}
%\begin{definition}{\textbf{Coverage rate:}}
%    Given a set of real-world data samples, coverage rate is the percentage of the real-world data samples which are bytes/mapping covered by data samples generated by proposed protocol fuzzing.
%\end{definition} 

{\bf Measuring the coverage rates. } 
To measure the coverage rates for the four network attacks, we have collected additional non-fuzzed data and measured the coverage rates with respect to the fuzzed data collected in Section~\ref{sec:data-gen}. The non-fuzzed data are collected by launching each kind of network attack with different parameters (e.g., IP addresses, MAC addresses, process names, etc.) for hundreds of times so that data collected in different attack sessions are not identical to each other.

We have measured the coverage rates for ARP poisoning, DNS cache poisoning, and TELNET session hijacking, respectively. 
Our results show that, for all the three network attacks, the coverage rates are all 100\%. 
In addition, we also assess the comprehensiveness of the training data generated for detecting PtH in 
an ad hoc way, and found that for each being-fuzzed field, 
every value observed in the non-fuzzed network packets
appeared at least once in the fuzzed data.   
% and the mapping coverage rate for PtH. 
In summary, our results show that a correlation between high detection accuracy and high coverage rates exists.



==> 7-detect_in_APT.tex <==
\section{APT Case Studies: Detecting Real-World Attacks}
\label{sec:APT_detection}

\begin{table*}
    \centering
        \caption{Four APT examples}
    \begin{tabular}{lllll}
    \hline
    APT name     & 1st technique           & 2nd technique            & 3rd technique       & 4th technique     \\ \hline
    APT\_EX1       & Supply chain attack     & Local data collection    & PtH       & Data exfiltration \\
    APT\_EX2       & Drive-by compromise     & ARP poisoning            & Supply chain attack & Data exfiltration \\
    APT\_EX3       & Drive-by compromise     & DNS cache poisoning      & Supply chain attack & Data exfiltration \\
    APT\_EX4       & Drive-by compromise     & TELNET session hijacking & Data exfiltration   & (None)            \\ \hline
    \end{tabular}
    \vspace*{1mm}
    \label{tab:APTs}
\end{table*}


%\subsection{Model usability}
In this section, we will prove that models trained with protocol fuzzing generated data can be used to identify real-world attacks. In another word, the models still perform well on non-fuzzed data. 
For this purpose, we have formed four APT examples, each containing one network attack discussed in section~\ref{sec:detect_with_NN}. Different from data in section~\ref{sec:detect_with_NN}, attacks in APT examples are launched without fuzzing. Therefore, if the models trained in section~\ref{sec:detect_with_NN} can still detect the corresponding attacks, then the effectiveness of the proposed approach in 
detecting real-world attacks is proved. 

The four APT examples are shown in Table~\ref{tab:APTs}, in which the four network attacks are used. The testbed of those four APTs is the same. It constructs a LAN that contains a router with, a Windows server hosting a Windows domain on the LAN, a local DNS server, two Windows user machines, and two Linux servers. We will explain 1) how each APT works
%and generates malicious impact on the affected enterprise networks
; 2) the role of the network attacks, and how identifications of those network attacks contribute to the detection of the whole APT.

\subsection{APT Descriptions}
\emph{APT\_EX1} contains four attacks, in which the first two are targeting the Windows server, and the last two target other Windows user machines. The attacker first gains initial access to the Windows server via supply chain attack and then collects local information such as other user accounts and credentials (hashes). Supply chain attacks means attackers embed malicious components into the hardware or software before it is delivered to the users so that they can compromise the system through the security hole later. With the collected local information, the attacker can launch PtH attack to access other Windows user machines of interest, and steal critical data through data exfiltration.

\emph{APT\_EX2} contains four attacks: the first one is against user machines; the second one is against the router and the Windows server; and the last two are against the Windows server. The attacker first gains initial access to a user machine using a drive-by compromise, such as drive by download. Later, the attacker can launch an ARP poisoning attack towards the router and the Windows server. The purpose is to intervene the network communications between the Windows server and the router, thus enabling supply chain attack. After the success of supply chain attack, the attacker gains access to the Windows server, so he/she can steal critical data by data exfiltration.

\emph{APT\_EX3} is mostly similar to APT\_EX2. In APT\_EX3, the second attack is replaced by DNS cache poisoning attack, which is against the local DNS server. The aim is to redirect the Windows server's network traffic to an attacker's chosen host, thus enabling supply chain attack towards the Windows server. The rest is the same as APT\_EX2.

\emph{APT\_EX4} contains three attacks, in which the first attack targets one user machine, and the last two target Linux servers. The attacker first gains initial access by drive-by compromise, then sniffs for TELNET sessions and try to hijack them to gain accesses to Linux servers. Finally the attacker can steal data of interest by data exfiltration.

%All the APTs above are launched respectively without fuzzing. 
%Necessary data for detection are collected separately.

\subsection{APT Detection}
All the individual attacks in Table~\ref{tab:APTs} can be identified. In Section~\ref{sec:detect_with_NN}, we have discussed the detection of PtH, ARP poisoning, DNS cash poisoning, and TELNET session hijacking, using our trained neural networks. The detection of the remaining attacks in Table~\ref{tab:APTs} using other approaches and tools such as intrusion detection systems, monitoring system logs or Windows Registry, and so on, is not the focus of this paper. Hence, we will skip the discussion on the detection of those attacks and only present how the detected individual attacks can be help the detection of APTs.  

%Hence, in this section, we'll skip those attacks and only discuss the remaining attacks in Table~\ref{tab:APTs} 

%Some of the attacks can be identified using our trained neural networks, which are described in Section~\ref{sec:detect_with_NN}. Below we will provide the details about other attacks.

%The supply chain attack is to manipulate products or product delivery mechanisms prior to receipt by a final consumer for the purpose of data or system compromise, such as manipulations to the development tools. The attack may be identified by scanning downloaded items with Anti-Virus (AV) products. Alternatively, network intrusion detection products like Snort \cite{Snort} can also detect it when the downloaded item tries to establish communication with the attacker's machine. Windows Defender can identify this technique and leave one entry in Windows event logs.

%In local data collection, the attacker needs to get data from the compromised machine for further intrusion, such as the user's password hashes for launching PtH attacks. This step usually requires two actions. One is to escalate the attacker's privilege to Administrator level, with which in the other action the attacker can interact with a system process, Local Security Authority Subsystem Service (LSASS), to get the hashes.

%In our experiments, the attacker bypasses Windows User Account Control (UAC) to escalate its privilege. Bypassing Windows UAC is a common privilege escalation technique towards Windows machines. Many procedures have been discovered to bypass UAC. An extensive list of available procedures can be found in the UACMe project \cite{UACMe}. Some procedures rely on modifying specific, user-accessible Windows Registry entries. Therefore, by monitoring accesses to the Registry with process monitor, especially entry creation and modification, bypassing UAC can be identified.

%After acquiring Administrator level privilege, the attacker does credential dumping to get hashes. Credential dumping is the process of obtaining account credentials, normally in the form of account names and password hashes. On a Domain Controller (DC), Active Directory (AD) service maintains all the users' account names and password hashes in the domain. They are stored in a database file locked by AD. Only some specific processes are allowed to access the contents of this file. Local Security Authority Subsystem Service (LSASS) is one of such special processes. It is given the right to read the database file because its role in a DC is to provide an interface for managing local security, domain authentication, and AD processes. With escalated privilege, attackers can craft queries, send them to LSASS, and get domain user account names and corresponding hashes. Therefore, we can monitor the LSASS process to identify this technique. We can either match some signatures in malicious queries or look for anomaly behaviors of LSASS to identify such hash dumping procedure.

%By data exfiltration, the attacker steals data of interest from the compromised machine and send them to the attacker-owned machine. Supposing that attackers are interested in sensitive data, system administrators can enforce disk I/O monitoring on sensitive files/folders on a machine. In this way, data exfiltration can be identified at disk level. Although this method may raise a lot of false positives, by correlating with identification results from previous attacks, we can correctly find out the access records left by the attacker.

From the APT descriptions in the previous subsection, it is easy to infer that underlying dependencies exist among attacks within one APT. Except the first attack step, a previous attack step enables the following attack step. For example, in APT\_EX1, without the initial access from supply chain attack, the attacker has no means to gather data; without the hashes got from local data collection, PtH cannot succeed; only after being able to move laterally to the target machine through PtH attack, the attacker can exfiltrate valuable data from the target machine. Therefore, after identifying each attack step, we can chain them together using such dependencies, so that the whole APT can be detected.

One method to chain two adjacent attacks in an APT is to check the process IDs in the two attacks. Generally, a malicious process created in the previous attack can be used to perform activities in the next attack. To chain the adjacent attacks, we may check if the process used in the later attack matches the malicious process or its child process in the previous attack. For example, in APT\_EX1, by supply chain attack, the attacker gains access to the Windows server, thus creating one malicious process for C\&C, which the attacker uses for the next step of local data collection. If the process ID (PID) involved in the local data collection is the same as the C\&C malicious process or its child process, these two attacks can be chained together. Similar approaches can be applied to chain the following attacks: 1) PtH and data exfiltration in APT\_EX1, supply chain attack and data exfiltration in APT\_EX2 and APT\_EX3, and TELNET session hijacking and data exfiltration in APT\_EX4; 2) Drive-by compromise and ARP poisoning in APT\_EX2, Drive-by compromise and DNS cache poisoning in APT\_EX3, and Drive-by compromise and TELNET session hijacking in APT\_EX4.  

The other chaining methods based on dependencies among attacks are discussed as follows:

\emph{Local data collection and PtH in APT\_EX1.} With local data collection, the attacker dumps the user accounts' password hashes to be used in PtH attacks. Therefore, if the user information leaked in local data collection is used for PtH, the local data collection and PtH can be chained together.

%Finally, the attacker create a malicious process at the end of PtH, and use the process or its child process for data exfiltration. If the process ID for the two stages match, the PtH and data exfiltration attacks can be chained together. 

%The final link between PtH and data exfiltration is similar to the first link, in which the attacker create a malicious process at the end of PtH, and use it, or its child process(es), for data exfiltration. Thus, a similar chaining rule can be applied to chain these two attacks together.

%\textbf{APT\_EX2}: First, we check if the process sending out malicious ARP packets for ARP poisoning matches the the process or child process created by drive-by compromise. If match, drive-by compromise and ARP poisoning will be chained together. 
%Through drive-by compromise, the attacker gains access to one user machine, thus creating one malicious process. The attacker then uses the malicious process or its child process to send out malicious ARP packets for ARP poisoning. If the PID of the process sending out malicious ARP packets is the same or a child process of that malicious process, it is safe to chain the two attacks together.

\emph{ARP poisoning and supply chain attack in APT\_EX2.} ARP poisoning attack is to trick the victim into a falsified mapping between IP addresses and MAC addresses. If the supply chain attack's victim has the IP addresses and/or MAC addresses in the ARP poisoning, we can chain ARP poisoning and supply chain attack together.

%Third, the supply chain attack and data filtration can be chained together similarly by checking if the process ID for C\&C and the ID for data exfiltration matches.   

%By supply chain attack, the attacker creates one malicious process on the Windows server for C\&C, which is used later for data exfiltration. Thus the two attacks can be chained by PID.

%\textbf{APT\_EX3}: The only difference between APT\_EX2 and APT\_EX3 is the second attack. Drive-by compromise and DNS cache poisoning can be chained by PID, which has been discussed earlier. 

\emph{DNS cache poisoning with supply chain attack in APT\_EX3.} To chain DNS cache poisoning with supply chain attack, the key is in the domain name. If the domain being poisoned appears in the download link in supply chain attack, then the two attacks can be chained together. 
%The third and forth technique can be chained in the same way as in APT\_EX2.

%\textbf{APT\_EX4}
%Drive-by compromise and TELNET session hijacking can be chained by PID, as discussed earlier. 
\emph{TELNET session hijacking attack and data exfiltration in APT\_EX4.} IP address is the key in this case to chain the TELNET session hijacking attack and data exfiltration on another machine. If the victim in the TELNET session hijacking attack is the same one as that of data exfiltration, then the two attacks can be chained together.

As what has already been shown in the literature~\cite{zou2020automatic}, individual attack identification results can be chained together by system objects dependencies as above to detect whole APTs. To detect the four APT examples above, we implemented the same framework. The inputs include network logs captured by Wireshark~\cite{wireshark}, Windows event logs, and process activity logs captured by Process Monitor~\cite{ProcessMonitor}. The output of the framework is a list of detected APTs in the order of completeness. Different APT examples produce different logs sets. Each log set belonging to different APTs are input into the framework respectively. All the four APTs are fully detected and put at the top of the list in the output of the framework. 
%For all the four APTs, and we observed that, in every output of the four cases, the corresponding APT is detected fully and put at the top of the list. 
That is, every individual step is successfully identified, and every couple of adjacent steps in the APTs is chained by system object dependencies.

As stated earlier, all attacks in our example APTs are launched without fuzzing, including the network attacks we discussed in section~\ref{sec:detect_with_NN}. This clearly indicates that models trained with fuzzed data can be used to detect real-world attacks (non-fuzzed data).

